Reframing Instructional Prompts to GPTk's Language

What kinds of instructional prompts are easier to follow for Language Models (LMs)? We study this question by conducting extensive empirical analysis that shed light on important features of successful instructional prompts. Specifically, we study several classes of reframing techniques for manual reformulation of prompts into more effective ones. Some examples include decomposing a complex task instruction into multiple simpler tasks or itemizing instructions into sequential steps. Our experiments compare the zero-shot and few-shot performance of LMs prompted with reframed instructions on 12 NLP tasks across 6 categories. Compared with original instructions, our reframed instructions lead to significant improvements across LMs with different sizes. For example, the same reframed prompts boost few-shot performance of GPT3-series and GPT2-series by 12.5% and 6.7% respectively averaged over all tasks. Furthermore, reframed instructions reduce the number of examples required to prompt LMs in the few-shot setting. We hope these empirically-driven techniques will pave the way towards more effective future prompting algorithms.

==> old_text.tex <==




%We study various techniques to \emph{reframe0} instructions to increase their efficacy when provided to language models (LM). 


% that could lead to successful results. Furthermore, we propose    of a  high-level attributes of successful task instructions (e.g., making them shorter, step-wise, etc.). 
% For instance, we observe that decomposing them into multiple simpler sub-steps often lead to performance improvements in the overall task.
%Guided by such empirical intuitions, we provide several types of prompt reframing techniques intended to be applied by model designers. 



\begin{comment}
The recent literature has shown promising results when prompting language model with task definition prompts. We study different areas where there are issues associated with prompting in GPT3 and provide \name{}- a class of guidelines to \emph{reframe} prompts and resolve the issues. Backed by extensive empirical analysis on GPT3, we observe several high-level attributes of successful task definition prompts.
For instance, we observe that decomposing task into multiple simpler tasks often lead to performance improvements in the overall task.
Guided by such empirical intuitions, we provide several types of prompt reframing techniques intended to be applied by model designers. 
We experiment over 12 tasks across 6 diverse categories (question generation, classification, etc.). 
Our results show that reframing improves few-shot learning performance by 14\% while reducing sample complexity over existing few-shot baselines. The performance gains are particularly important on large language models, such as GPT3 where tuning models or prompts on large datasets is not feasible. Furthermore, we observe that such gains are not limited to GPT3; the reframed tasks remain superior over raw instructions across different model architectures, underscoring the cross-model generality of these guidelines. We hope these empirical-driven techniques will pave way for more effective ways to prompt LMs in future. 
\end{comment}



\hanna{I think it is better to directly start with prompting... why do we need to start with tuning?} Tuning pre-trained language models (LM) to particular datasets has lead to major progress across a broad range of tasks~\cite{seo2017bidaf,khashabi2020unifiedqa,aghajanyan2021muppet}. Despite their success, these algorithms are prohibitively expensive for large scale language models such as GPT3~\cite{brown2020gpt3} that involve gradient computations on large-scale datasets. 

\hanna{(1) define prompting and say that it has shown successful results in a few tasks. (2) it is unstable, (3) people have shown calibration or prompt engineering, and write down one/two issue with each. (4) Here, what do we do? we study issues with different types of prompts and introduce reframing}



The recent approaches~\cite{liu2021promptingsurvey}  provide large LMs with natural language {\it prompts} and enable strong few-shot baselines while being interpretable~\cite{schick2020few,le-scao-rush-2021-many,tam2021improving}, 
containing instructions and a few training examples and provide them to large LMs to 
Despite such benefits finding effective language prompts has been under-explored, 
except for a narrow range of tasks such as in-filling~\cite{jiang2020whatmodelsknow} or classification~\cite{schick2021exploiting, lu2021fantastically}.

\hanna{Here, explain that gpt3 is unstable with different types of prompts, people have looked at prompt engineering which is mainly changing prompts at surface-level}
While existing techniques for prompt engineering \cite{petroni2019language, schick2020few, schick2021exploiting} involves rearranging the original prompt and generating prompts that have a lot of word overlap with the original prompt, \emph{reframing} has a much wider scope as it often involves generating prompts that have a very few word overlap with the original prompt. The guidelines we provide are intended to bridge gaps in the prompt engineering literature such as their applicability within a narrow range of tasks and absence of illustrative use cases to guide designers in engineering prompts.
% prompting via examples~\cite{}. 
%Moreover, there does not exist a concrete guideline to manually design prompts.\daniel{not sure what this last sentence is adding to the earlier sentence. }


We understand different areas where there are issues associated with prompting in GPT3 and provide \name{}- a class of guidelines to \emph{reframe} prompts and resolve the issues.
We observe that humans usually use high-level instructions, but these are not machine-friendly, as evidenced by lower performance of models in response to such Instructions. In pursuit of resolving the issues, we provide \name{}- a class of guidelines for model designers to \emph{reframe} prompts. This contains 5 types of \emph{reframing} techniques to reduce task difficulty: for example by decomposing a task into multiple sub tasks and by providing crisp and concrete instructions that are free of domain specific keywords. We provide illustrative use-cases associated with each type of \emph{reframing} techniques. Figure~\ref{fig:fig1}-left shows an example for writing questions that require entity coreference~\cite{dasigi2019quoref}.
GPT3 has difficulties solving the original task based on its definition which were originally provided to the humnan annotators of the dataset \cite{mishra2021natural} (the yellow box at the top). However, it succeeds when the task gets decomposed to four simpler and easier sub-tasks.

We experiment over 12 tasks across 6 diverse categories in Natural Instructions \cite{mishra2021natural}. Our results (\S\ref{sc:experiments}) show that \emph{reframing} improves average few-shot learning performance by 17\% and notably improve sample complexity over raw instructions (which were originally designed for humans). We also observe evidence for cross-model generalization since \emph{reframing} performed for GPT3 gets transferred to other models (Figure \ref{fig:fig1}-right red line shows considerable performance improvement over original task instructions i.e. without reframing (blue line)); this is in contrast to fine-tuning and prompt-tuning which need to be performed separately for each model. The finetuning baselines with GPT2Large are much lower than the performance of GPT3-Instruct with \emph{reframing}, indicating that it is more effective for a model designer to reframe a task for GPT3-Instruct than performing fine-tuning for a smaller model like GPT2Large with 200x more data.

\name{} is intended to fasten model development as model designers can come up with new reframed tasks in a matter of minutes, in contrast to the expensive data curation process for a new task. However, on the down side, reframing at its current form is not automatic and require humans.
Hence, there is opportunity to develop an algorithmic solution to reframe tasks. We expect our study will lead to develop better few-shot learning models, prompting techniques and the capability to perform cross-model generalization that has remained unexplored in the literature. We believe this direction will redirect more attention on investigating ways of better using large scale language models, thereby maximizing the benefits we can reap from the investments already poured in to create such models.

\textbf{Contributions:} 
(a) We understand different areas where there are issues associated with prompting in GPT3 and provide \name{}- a class of guidelines to simplify prompts and resolve the issues. 
(b) Guided by empirical intuitions on GPT3, we propose 5 types of \emph{reframing} techniques aimed to be applied by model designers. We provide illustrative use-cases associated with each type of \emph{reframing} technique. 
(c) Experiments on diverse tasks show that \emph{reframing} gives rise to superior few-shot learning performance, improves sample complexity over raw instructions and shows evidence for cross-model generalization. On a broader level, our study provides insights on potential ways to better use machines by maximizing the benefits we can reap from the investments already poured in to create large scale language models. 


\begin{comment}
\daniel{
% Our analysis falls under the general umbrella of \emph{prompt-engineering}~\cite{liu2021promptingsurvey}. 
% The existing work in this dire in this a narrow range of tasks such as in-filling~\cite{jiang2020whatmodelsknow} or classification~\cite{schick2021exploiting, lu2021fantastically}.

% While existing techniques for prompt engineering \cite{petroni2019language, schick2020few, schick2021exploiting} involves rearranging the original prompt and generating prompts that have a lot of word overlap with the original prompt, \emph{reframing} has a much wider scope as it often involves generating prompts that have a very few word overlap with the original prompt. The guidelines we provide are intended to bridge gaps in the prompt engineering literature such as their applicability within a narrow range of tasks and absence of illustrative use cases to guide designers in engineering prompts.


Here we need a paragraph to define how it's related to other work: 
 - It falls under the general family of prompt engineering
 - It is related to and inspired by several recent works 
 - However, these works often target a niche problem 
    - and their algorithms are also specific to that pronlem 
 - While it is not algorithmic, we investigate a broader range of tasks. 
}


The recent approaches~\cite{liu2021promptingsurvey}  provide large LMs with natural language {\it prompts} and enable strong few-shot baselines while being interpretable~\cite{schick2020few,le-scao-rush-2021-many,tam2021improving}, 
containing instructions and a few training examples and provide them to large LMs to 
Despite such benefits finding effective language prompts has been under-explored, 
except for a narrow range of tasks such as in-filling~\cite{jiang2020whatmodelsknow} or classification~\cite{schick2021exploiting, lu2021fantastically}.

While existing techniques for prompt engineering \cite{petroni2019language, schick2020few, schick2021exploiting} involves rearranging the original prompt and generating prompts that have a lot of word overlap with the original prompt, \emph{reframing} has a much wider scope as it often involves generating prompts that have a very few word overlap with the original prompt. The guidelines we provide are intended to bridge gaps in the prompt engineering literature such as their applicability within a narrow range of tasks and absence of illustrative use cases to guide designers in engineering prompts.
% prompting via examples~\cite{}. 
%Moreover, there does not exist a concrete guideline to manually design prompts.\daniel{not sure what this last sentence is adding to the earlier sentence. }
\end{comment}


% On a broader level, we hope this work motivates out-of-the-norm approaches to exploiting the knowledge harnessed by massive LMs. 
% our study provides insights on potential ways to better use machines by maximizing the benefits we can reap from the investments already poured in to create large scale language models. 



How can model designers turn task instructions into  effective prompts for language models? Backed by extensive empirical analysis on GPT3, we observe important features for successful instructional prompts, and propose several reframing techniques for model designers to create such prompts. For example, a complex task can be decomposed into multiple simpler tasks. We experiment over 12 NLP tasks across 6 diverse categories (question generation, classification, etc.). 
Our results show that reframing improves few-shot learning performance by 14\% while reducing sample complexity over existing few-shot baselines. The performance gains are particularly important on large language models, such as GPT3 where tuning models or prompts on large datasets is not feasible. Furthermore, we observe that such gains are not limited to GPT3; the reframed tasks remain superior over raw instructions across different model architectures, underscoring the cross-model generality of these guidelines. We hope these empirical-driven techniques will pave way for more effective ways to prompt LMs in future.


% The fine-tuning baselines with  are much lower than the performance of GPT3-Instruct with \name{}, % indicating that it is more effective for a model designer to reframe a task for GPT3-Instruct (red line) than performing fine-tuning for a smaller model like GPT2Large (green line) with 200x more data.
%give examples
% oringial task is not undestandable by persons
% what does original task mean?
% repeation principle is getting violated in enforcment reframing

% \daniel{I think we need to: "descriptive" --> "instructional"}


%Overall, we believe that prompt reframing can be an effective approach for fast model development, particular in the world of massive LMs that might not be easy to fine-tuned. 

% , in contrast to the expensive data curation process for a new task. However, on the down side, reframing at its current form is not automatic and require humans.
% Hence, there is opportunity to develop an algorithmic solution to reframe tasks. 

% prompting techniques and the capability to perform cross-model generalization that has remained unexplored in the literature. 
% We believe this direction will redirect more attention on investigating ways of better using large scale language models, thereby maximizing the benefits we can reap from the investments already poured in to create such models.


%In particular, there is little understood about what instructions tend to be more effective for LMs and furthermore, how can an average user of LMs 
%find
% describes
%them.\daniel{not fully happy with this last sentence. Thoughts?}

% this is the modular qa work. Instead of using model, annotation, just give it to GPT3.
%make it for decomposition only
% instead of making it work for constrained setup where the task is to answer question from a context (the reason we did not select is because this can be done in the constraint reframing setup).
% \subsubsection{\textsc{Exemplar Reframing}}
% \textbf{Motivation} Models hardly generate an answer type different from the answer type of examples provided along with the prompt. \\
% % This biases model prediction to the answer types present in the examples associated with the prompt. \\
% \textbf{Definition} We add diverse answer types \ref{cp6} and provide model the exposure to a relatively larger answer space.\\
% \textbf{Example} Table \ref{tab:reframing examples} (row1) illustrates a question-answering task on transient vs stationary events from the MCTaco \cite{zhou2019going} dataset. The raw task contains an example with answer type ``hour''. GPT3 in response to various questions generates answers mostly in the form of some ``hours'', even though this is an an open-ended answer generation task. In the reframed task, we provide GPT3 the exposure to various forms of answer types. This improves GPT3's response and it also learns to generate similar answer types such as ``weeks''.
% % Table \ref{tab:reframing examples6_7}-row1 illustrates Exemplar Reframing where the task is a question-answering task on transient vs stationary events from the MCTaco \cite{zhou2019going} dataset. This is an open-ended answer generation tasks and model response can be anything. However, if we provide one example with answer type in ``hour'' (column-1), GPT3 produces answers mostly in the form of some ``hours''. In the reframed task (column-2), we provide GPT3 the exposure to various forms of answer types which are ``hours'', ``years'', ``minutes'', ``seconds'' and ``months''. This improves GPT3's response and it also learns to generate similar answer types such as ``weeks''.
% % Several other types of examples reframing have also been performed in a few recent works \cite{zhao2021calibrate, lu2021fantastically}.

% \subsubsection{\textsc{Parameter Reframing:}}
% % \daniel{this does not quite fit the definition of "reframing" (which is expected to be applied to the input instructions). }
% % \swaroop{I agree, this is sort of a task-reframing where instead of using natural language to instruct models, we use paramters, since these are readily available. E.g. temperatue 1 can be stated as "Generate diverse texts" and temperature 0 as "stick to the instructions and do not be creative". \textbf{Futuristic idea}: The automation of \name{} might require to make a lot of parameters which later can be controlled instead of adding all these in natural langugage}
% \textbf{Motivation} Default parameters of GPT3 is not always ideal for every task. For example, the default temperature which is on the higher side is not suitable for a task where we don't want diversity.\\
% % default temperature is usually high, however higher temperature results in diverse content which is not suitable for say a question answering task where the answer lies in the passage or a task to find out overlapping word between two sentences.\\
% \textbf{Definition} Select the parameters:  engine, temperature, stopping condition, model, output token size \etc{} based on the task requirements. For example if the task does not require any creativity and a fine-grained control is necessary, keep temperature close to 0, whereas if the task demands diversity, keep it close to 1 if the task demands diversity. \\
% % This is the easiest form of reframing in GPT3.
% \textbf{Example} Table \ref{tab:reframing examples} (row2) illustrates a task where the goal is to generate a plan. With default parameters, GPT3 usually produces some text (often in the form of a conversation) that are not coherent and relevant enough to form a plan. However, on appropriately setting parameters by increasing output token size, controlling temperature, changing engine, stop condition and the underlying model, GPT3's response improves.

% \begin{table}[t]
%     \centering
%     \small
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{ccc}
%         \toprule
%         task & source & category    \\
%         \midrule
%         \makecell{generating questions\\ on event duration} & \makecell{MC-TACO \\ \cite{zhou2019going}} & \multirow{3}{*}{\makecell{Question  \\ Generation\\  (QG) }}   \\ 
%         \cmidrule{1-2}
%         \makecell{generating questions\\ on sentence composition } & \makecell{QASC \\ \cite{khot2020qasc}} & \\ 
%         \midrule
%         \makecell{answering event \\ coreference  questions} & \makecell{Quoref \\ \cite{dasigi2019quoref}} & \multirow{3}{*}{\makecell{Answer\\Generation \\ (AG)}}   \\ 
%         \cmidrule{1-2}
%         \makecell{answering fill in the \\blank questions on\\ coreference resolution} & \makecell{WinoGrande \\ \cite{sakaguchi2020winogrande}} & \\ 
%         \midrule
%         \makecell{identifying inappropriate \\ content in context} & \makecell{CosmosQA \\ \cite{huang2019cosmos}} & \multirow{3}{*}{\makecell{Classification \\ (CF)}}   \\ 
%         \cmidrule{1-2}
%         \makecell{identifying bad questions\\ in reading comprehension} & \makecell{MultiRC \\ \cite{khashabi2018looking}} &  \\ 
%         \midrule
%         \makecell{generating incorrect \\ answers to event \\  transience questions} & \makecell{MC-TACO \\ \cite{zhou2019going}} & \multirow{3}{*}{ \makecell{Incorrect \\ Answer \\ Generation \\  (IAG)} }   \\ 
%         \cmidrule{1-2}
%         \makecell{generating incorrect  \\ answers  to event \\  duration questions} & \makecell{MC-TACO \\ \cite{zhou2019going}} & \\ 
%         \midrule
%         \makecell{modifying fill in the\\ blank questions on\\ coreference resolution} & \makecell{WinoGrande \\ \cite{sakaguchi2020winogrande}} & \multirow{3}{*}{\makecell{Text \\ Modification \\ (MM)}}   \\ 
%         \cmidrule{1-2}
%         \makecell{generating paraphrase\\ of given sentences} & \makecell{Miscellaneous \\ } & \\ 
%         \midrule
%         \makecell{finding overlapping words\\ between two sentences} & \makecell{QASC \\ \cite{khot2020qasc}} & \multirow{3}{*}{\makecell{Verification \\ (VF)}}   \\ 
%         \cmidrule{1-2}
%         \makecell{Identifying words\\ essential for choosing\\ correct answers.} & \makecell{Essential-Terms \\ \cite{khashabi2017learning}} & \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{List of evaluation tasks used in this study (\S\ref{sc:experiments}).  }
%     \label{tab:tasks}
% \end{table}


% \textsc{Pattern Reframing} and \textsc{Specialization reframing} are most commonly used. However, all types of reframings are found to be effective across various categories. 

% We observe that there exists a correlation between the task category and the reframing techniques as our results show that certain reframing types are dominant on tasks of certain categories. \textsc{Pattern Reframing} is dominant for Question Generation and Incorrect Answer Generation tasks, \textsc{Specialization Reframing} is most effective for Answer Generation, Minimal Text Modification and Verification tasks. Similarly, \textsc{Restraining Reframing} and \textsc{Itemizing Reframing} contributes the most in case of Classification and Long Text Generation tasks respectively.
% \subsubsection{Effect of Reframing on Reasoning Skills}

% \footnote{Note that not all reframing techniques are effective for a particular task. }
% Hence, we do not conduct experiments with every pair of reframing techniques and tasks and evaluate the performance gain associated with each of the reframing techniques. 
% The numbers associated with the rerframing techniques show the average performance gain associated with each of the reframing techniques on being applied to tasks of various categories.

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}{0.50\textwidth}
%         \centering
%         \includegraphics[scale=0.7, trim=1.5cm 1cm 1cm 1cm]{img/intro-fig-1.pdf}
%         \caption{GPT3 has difficulty in writing questions that require entity coreference resolutions based on a single lengthy prompt (top, in \yellowtext{yellow}),
%         however, it succeeds in solving a \emph{reframed} task that has four simpler sub-steps (bottom, in \greentext{green}).}
%      \label{fig:fig1a}
%     \end{subfigure}%
%     \hspace{.2cm}
%     \begin{subfigure}{0.46\textwidth}
%         \centering
%         \includegraphics[scale=0.52, trim=0.7cm 0cm 0cm 0cm]{img/chartmodel.pdf}
%         \caption{
%         Across a variety of model sizes, {\color{red}reframed prompts} consistently show considerable performance gain over {\color{blue} raw task instructions (no reframing)} \changed{in a few-shot learning setup}. 
%         % Cross-model generalization across several models in the GPT-Series. 
%         % \name{} (red line) results in considerable performance improvement over original task instructions i.e. without reframing (blue line) across all models. 
%         Since fine-tuning GPT3 is prohibitively expensive, we show the performance of fine-tuning smaller models ({\color{darkgreen}horizontal} {\color{orange} lines}). 
%         % For comparison, we show the performance of fine-tuning , 
%         This results indicates that
%         \changed{
%             % for a fixed compute budget, 
%             \emph{evaluating} reframed prompts on a large model like GPT3-instruct (red line) might be more effective that \emph{fine-tuning}} a smaller model like GPT2Large (green line) with 200$\times$ more data.
%             % This results indicates that it might be more effective for a model designer to reframe a task prompt for a large model like GPT3-instruct (red line) than performing fine-tuning for a smaller model like GPT2Large (green line) with 200$\times$ more data.
%             Details of the experiments in \S\ref{sc:experiments}. 
%         }
%         \label{fig:fig1b}
%     \end{subfigure}
%     \caption{(a) An example reframing. 
%     % Illustration of a type of \name{}. 
%     (b) A summary of the empirical results. 
%     % in this workthe cross-model generalization results associated with \name{}
%     }
%     % \label{fig:fig1}
% \end{figure*}



% \subsubsection{\textsc{Pattern Reframing}}
% \subsubsection{\textsc{Itemizing Reframing}}
% \subsubsection{\textsc{Decomposition Reframing}}
% \subsubsection{\textsc{Restraining Reframing}}
% \subsubsection{\textsc{Specialization Reframing}}

\input{appendix_examples_pattern}
% \begin{table*}[h]
%     \small
%     \centering
%      \resizebox*{!}{0.72\textheight}{%
%     \begin{tabular}{p{16.5cm}}
%         \toprule
%         \textit{Raw task definitions and their \textsc{\textcolor{purple}{Pattern Reframed}} counterpart} \\ 
%         \midrule
%         \textcolor{brown}{\textit{\textbf{Raw Task:}}} \textit{Craft a question which requires commonsense to be answered. Based on the given context, craft a common-sense question, especially those that are LONG, INTERESTING, and COMPLEX. The goal is to write questions that are easy for humans and hard for AI machines! To create such questions, here are some suggestions: A. What may (or may not) be the plausible reason for an event? B. What may (or may not) happen before (or after, or during) an event? C. What may (or may not) be a plausible fact about someone (or something)? D. What may (or may not) happen if an event happens (or did not happen)? You can also create other types of question.} \newline \textbf{Context}:I was told, in person over the phone, that my shoes were on their way. They have my money. I have no shoes. \newline \textbf{Question}: \textcolor{red}{What may be the plausible reason for this event?}\\
%         \cdashlinelr{1-1}
%         \textcolor{brown}{\textit{\textbf{Reframed Task:}}}
%         \textit{Use 'what may happen', 'will ...?', 'why might', 'what may have caused', 'what may be true about', 'what is probably true about', 'what must' and similar phrases in your question based on the input context.}\newline \textbf{Context}:I was told, in person over the phone, that my shoes were on their way. They have my money. I have no shoes. \newline \textbf{Question}:\textcolor{blue}{What may happen if my shoes never show up?}\\ [0.1cm]
%         \midrule
%         \midrule
%         \textcolor{brown}{\textit{\textbf{Raw Task:}}} \textit{Craft a question which requires commonsense to be answered. Based on the given context, craft a common-sense question, especially those that are LONG, INTERESTING, and COMPLEX. The goal is to write questions that are easy for humans and hard for AI machines! To create such questions, here are some suggestions: A. What may (or may not) be the plausible reason for an event? B. What may (or may not) happen before (or after, or during) an event? C. What may (or may not) be a plausible fact about someone (or something)? D. What may (or may not) happen if an event happens (or did not happen)? You can also create other types of question.} \newline \textbf{Context}:you see , at my age relationship is kind of important and i thought i got the one after all these years . I noticed that once again i was wrong . i was good simply because i was good , i was caring , helping , supportive , bla bla blaaa . \newline \textbf{Question}: \textcolor{red}{what is the reason why you keep falling for the same type of person?\newline \newline
%         A. What is the reason you keep falling for the same type of person?\newline
%         B. What may (or may not) be the problem with your relationships?\newline
%         C. What may (or may not) be the possible cause}\\
%         \cdashlinelr{1-1}
%         \textcolor{brown}{\textit{\textbf{Reframed Task:}}}
%         \textit{Use 'what may happen', 'will ...?', 'why might', 'what may have caused', 'what may be true about', 'what is probably true about', 'what must' and similar phrases in your question based on the input context.}\newline \textbf{Context}:you see , at my age relationship is kind of important and i thought i got the one after all these years . I noticed that once again i was wrong . i was good simply because i was good , i was caring , helping , supportive , bla bla blaaa . \newline \textbf{Question}:\textcolor{blue}{What may happen if i don't get the one i want ?}\\ [0.1cm]
%         \midrule
%         \midrule
%         \textcolor{brown}{\textit{\textbf{Raw Task:}}} \textit{Craft a question which requires commonsense to be answered. Based on the given context, craft a common-sense question, especially those that are LONG, INTERESTING, and COMPLEX. The goal is to write questions that are easy for humans and hard for AI machines! To create such questions, here are some suggestions: A. What may (or may not) be the plausible reason for an event? B. What may (or may not) happen before (or after, or during) an event? C. What may (or may not) be a plausible fact about someone (or something)? D. What may (or may not) happen if an event happens (or did not happen)? You can also create other types of question.} \newline \textbf{Context}: GPS technology dates back to the time when first ever satellite was launched in the sky in 1979. The era of global positioning started then. \newline \textbf{Question}: \textcolor{red}{What was the first satellite launched in 1979? \newline \newline
%         A. Voyager 1 \newline
%         B. Voyager 2 \newline
%         C. Pioneer 11 \newline
%         D. Pioneer 10}\\
%         \cdashlinelr{1-1}
%         \textcolor{brown}{\textit{\textbf{Reframed Task:}}}
%         \textit{Use 'what may happen', 'will ...?', 'why might', 'what may have caused', 'what may be true about', 'what is probably true about', 'what must' and similar phrases in your question based on the input context.}\newline \textbf{Context}:GPS technology dates back to the time when first ever satellite was launched in the sky in 1979. The era of global positioning started then. \newline \textbf{Question}:\textcolor{blue}{Why might GPS technology have been invented??}\\
%         \bottomrule
%         \end{tabular}
%         }
%         \caption{
%             Examples of {\bf Pattern Reframed} instructions. 
%             \textit{Italicized} text represents the instructions. 
%             GPT's response to the raw and refraned instructions are indicated with \textcolor{blue}{blue} and \textcolor{red}{red} markings, respectively.
%         }
%     \label{tab:pattern_reframing_both1}
% \end{table*}

